Relativistic mean-field theory applied to the study of neutron star properties

Nuclear physics can be applied in various ways to the study of neutron stars. This thesis reports on one such application, where the relativistic mean-field approximation has been employed to calculate the equations of state of matter in the neutron star interior. In particular the equations of state of nuclear and neutron star matter of the NL3, PK1 and FSUGold parameter sets were derived. A survey of available literature on neutron stars is presented and we use the derived equations of state to reproduce the properties of saturated nuclear matter as well as the mass-radius relationship of a static, spherical symmetric neutron star. Results are compared to published values of the properties of saturated nuclear matter and to available observational data of the mass-radius relationship of neutron stars.

==> chapterQHD.tex <==
\chapter{Quantum Hadrodynamics}\label{QHD}
general intro oor hoe nuclear force model - exchange of mesons (soek review article - Meng?, check ook QHD folder in M-artikels) en skryf dit so dat die verskillende models ook motiveer of motiveerbaar maak.
%
%
%
\section{Quantum Hadrondynamics 1}\label{QHD1}
Quantum Hadrondynamics 1 (QHD1), also known as the $\sigma$ - $\omega$ model, is the simplest model of the Walecka-type models. It models the nuclear force by the exchange of neutral scalar ($\sigma$) and neutral vector ($\omega$) mesons. Thus the nucleon-nucleon interaction is described by three fields, baryon-, scalar meson- and vector meson-fields. Since no charged mesons are included in the model, the baryons are assumed to be neutral and therefore no distinction is made between neutrons and protons in QHD1. (QHD2, which includes the charged $\pi$-meson,pion, will be sensitive to the different charged baryons.) The Lagrangian of QHD1 is given the following (in natural units):
\begin{eqnarray}
		{\cal L} = \bar{\psi}(x)[\gamma_{\mu}(i\partial^{\mu}-g_{v}V^{\mu}) - (M-g_{s}\phi)]\psi(x) +
		 \frac{1}{2}(\partial_{\mu}\phi\partial^{\mu}\phi - m_{s}^{2}\phi^{2}) - 
		 \frac{1}{4}V_{\mu\nu}V^{\mu\nu} + \frac{1}{2}m_\omega^{2}V_{\mu}V^{\mu}\nonumber
\end{eqnarray}
where
\begin{itemize}
\item $V$ denotes the vector meson field,
\item $\phi$ denotes the scalar meson field,
\item $m_\omega$ and $m_s$ the different meson masses and $M$ denotes the baryon mass,
\item $g_{v}$ and $g_{s}$ the vector and scalar couping constants and 
\item $V_{\mu\nu} = \partial_{\mu}V_{\nu} - \partial_{\nu}V_{\mu}$.
\end{itemize}
The Lagrangian is a Lorentz scalar and has the dimension of fm$^{-4}$.\\
\\
In constructing the Lagrangian it was assumed that the neutral scalar mesons couples to the scalar density of the baryon field and that the neutral vector mesons couples to the conserved baryon current \cite{walecka}.\\
\\
Using the Euler-Lagrange equations the equations of motion of the different fields can be constructed (!reference to chapter 2!).
%\begin{center}
	\begin{eqnarray}
		(\partial_{\mu}\partial^{\mu} + m_{s}^{2})\phi = g_{s}\bar{\psi}(x)\psi(x)\label{scalarEQM} \\
		\partial_{\mu}F^{\mu\nu} + m_\omega^{2}V^{\nu} = g_{v}\bar{\psi}(x)\gamma^{\nu}\psi(x)\label{bosonEQM} \\
		(\gamma_{\mu}(i\partial^{\mu}-g_{v}V^{\mu}) - (M-g_{s}\phi))\psi(x) = 0\label{baryonEQM}
	\end{eqnarray}
%\end{center}
Equation (\ref{scalarEQM}) is analogues to the equation of free scalar (field?) particles, the Klein-Gordon equation (\ref{KGE}), but in the case of (\ref{scalarEQM}) there is a source term that describes the coupling of the scalar particles to the scalar density of the baryons.\\
\\
Equation (\ref{bosonEQM}) is analogues to the Proca equation, with the coupling of the boson field to the conserved baryon current introduced in the source term ({\bf wat is 'n source term??})\\
\\
The equation of motion of the baryon field is the Dirac equation (\ref{DE}) with modified mass (due to the scalar field) and interaction with the vector field introduced in {\em minimal fashion}\\
\\
!From the formalism discussed in chapter(\ref{mechanics}) the energy-momentum tensor for QHD1 can be constructed.!(besluit of jy soos in JDW die formalisme uiteen wil sit)
Since equation (\ref{scalarEQM} - \ref{baryonEQM}) are non-linear, coupled equations they would be very difficult to solve and is therefore approximated in the {\em relativistic mean-field approximation}.
%
%
%
\subsection{Relativistic Mean-Field theory}\label{RMF}
In other quantum mechanical theories perturbation expansion of the coupling strenghts are used to approximate complicated equations. Within the framework of QHD the coupling strengths might be large and thus higher-order perturbative approximations will diverge. Also within the context of dense nuclear systems an approximation that is increasingly valid as the high-density limit would be preferable.\\
\\
In the relativistic mean-field approximation the value of the scalar and vector meson fields are replace by their groundstate expectation values. 
%\begin{center}
	\begin{eqnarray}
		\phi \longrightarrow \left\langle \phi\right\rangle = \phi_{0}\nonumber\\
		V_{\mu} \longrightarrow \left\langle V\right\rangle = \delta_{\mu 0}V_{0}\nonumber
	\end{eqnarray}
%\end{center}
The spatial components of the vector (omega meson) field vanish when the ground state of uniform static nuclear matter is considered, since the baryon current also vanishes in this case \cite{walecka},\cite{csg}.\\
\\
In the mean-field approximation the equations of motion of the different fields reduce to
%\begin{center}
	\begin{eqnarray}
		 m_{s}^{2}\phi_{0} = g_{s}\left\langle\bar{\psi}\psi\right\rangle\nonumber \\
		 m_\omega^{2}V_{0} = g_{v}\left\langle\bar{\psi}\gamma_{0}\psi\right\rangle\nonumber\\
		\gamma_{\mu}(i\partial^{\mu} - (M-g_{s}\phi_0))\psi = 0. \nonumber
	\end{eqnarray}
%\end{center}
Thus giving $\phi_{0}$ and $V_{0}$ as,
%\begin{center}
	\begin{eqnarray}
		 \phi_{0} = \frac{g_{s}}{m_{s}^{2}}\left\langle\bar{\psi}\psi\right\rangle\label{sigma0} \\
		 V_{0} = \frac{g_{v}}{m_\omega^{2}}\left\langle\psi^{\dagger}\psi\right\rangle = \frac{g_{v}}{m_\omega^{2}}\rho_{B}\label{omega0}
	\end{eqnarray}
%\end{center}
The Lagragian and energy-momentun tensor of QHD1 in the mean-field approximation thus reduces to
%\begin{center}
	\begin{eqnarray}
			{\cal L}_{MFT} = \bar{\psi}[i\gamma_{\mu}\partial^{\mu}-g_{v}\gamma^{0}V_{0} - (M-g_{s}\phi_{0})]\psi +
		 \frac{1}{2}m_{s}^{2}\phi_{0}^{2} - \frac{1}{2}m_\omega^{2}V_{0}^{2}\nonumber
	\end{eqnarray}
%\end{center}
From the above Lagrangian density the energy-momentum tensor of QHD1 in the mean-field approximation can be constructed and is given by
%\begin{center}
	\begin{eqnarray}		 
		 (T_{\mu\nu})_{MFT} = i\bar{\psi}\gamma_{\mu}\partial^{\nu}\psi - \frac{1}{2}( m_\omega^{2}V_{0}^{2} -
		  m_{s}^{2}\phi_{0}^{2}).\nonumber
	\end{eqnarray}
%\end{center}
From ({\bf ref na Lagrange Mech}) the energy density and pressure is given by,
\begin{eqnarray}
	\epsilon = \frac{1}{2}m_{s}^{2}\phi_{0}^{2} + 	\frac{1}{2}m_\omega^{2}V_{0}^{2} + 
							\frac{\gamma}{(2\pi)^{3}}\int^{k_{f}}_{0}d^{3}k\,\sqrt{k^{2} + (m - g_{s}\phi_{0})^{2}}\label{eps1}\\
	p = -\frac{1}{2}m_{s}^{2}\phi_{0}^{2} + 	\frac{1}{2}m_\omega^{2}V_{0}^{2} + 
							\frac{1}{3}\left(\frac{\gamma}{(2\pi)^{3}}\int^{k_{f}}_{0}d^{3}k\frac{k^{2}}{\sqrt{k^{2} +
							 (m - g_{s}\phi_{0})^{2}}}\right)\label{pres1}
\end{eqnarray}
and
\begin{itemize}
	\item$k_{f}$ denotes the fermi-wavemomentum of the highest occupied state and
	\item $\gamma$ is the degeneracy of the state.
\end{itemize}	
By defining the reduced mass, $m^{*}$ as
\begin{eqnarray}
	m^{*} \equiv m - g_{s}\phi_{0}\label{m*},
\end{eqnarray}
and imposing spherical symmetry, (\ref{eps1}) and (\ref{pres1}) can be re-written as
\begin{eqnarray}
	\epsilon &=& \frac{1}{2}m_{s}^{2}\phi_{0}^{2} + 	\frac{1}{2}m_\omega^{2}V_{0}^{2} + 
							\frac{\gamma}{2\pi^{2}}\int^{k_{f}}_{0}dk\,k^{2}\sqrt{k^{2} + {m^{*}}^{2}}\label{eps}\\
	p &=& -\frac{1}{2}m_{s}^{2}\phi_{0}^{2} + 	\frac{1}{2}m_\omega^{2}V_{0}^{2} + 
							\frac{1}{3}\left(\frac{\gamma}{2\pi^{2}}\int^{k_{f}}_{0}dk\frac{k^{4}}{\sqrt{k^{2} + {m^{*}}^{2}}}\right)\label{pres}						
\end{eqnarray}
To solve (\ref{eps}) or (\ref{pres}) values for $V_{0}$ and $\phi_0$ (and thus $m^{*}$) need to be obtained. $V_{0}$ can be
 solved quite easily in terms of the baryon density, $\rho_{B}$, by equation (\ref{omega0}) . The baryon density is defined as
\begin{eqnarray}
	\rho_{B} = \frac{\gamma}{(2\pi)^{3}}\int^{k_{f}}_{0}d^{3}k = \frac{\gamma}{6\pi^{2}}k_{f}^{3}\nonumber.
\end{eqnarray}
The solutions for $\phi_{0}$ (or $m^{*}$) can be obtained by minimizing the energy density with respect to $\phi_{0}$ (or $m^{*}$) \cite{walecka}.
By following this procedure for $m^{*}$ the following self-consistent equation is obtained:
\begin{eqnarray}
	m^{*} = m - \frac{g_{s}^{2}}{m^{2}_{s}}\frac{\gamma}{(2\pi)^{3}}\int^{k_{f}}_{0}d^{3}k 
					\frac{m^{*}}{\sqrt{k^{2} + {m^{*}}^{2}}}\nonumber \ .
\end{eqnarray}
By solving for $m^{*}$ the value for $\sigma_{0}$ is yielded by (\ref{m*}) and the energy density and the pressure can be solved for a specific value
 of $k_{f}$.\\
\\
NOu kan ons maar resultate in sit of QHD11 doen...
\\
\subsection{Observables of nuclear matter in QHD1}
\subsubsection{Symmetry energy}
To calculate the symmetry coefficient, $a_4$, given by 
\[
		a_{4} = \frac{1}{2}\left(\frac{\partial^{2}}{\partial t^{2}}\frac{\epsilon}{\rho}\right)_{t=0}\ \ \ \ \  \left(t\equiv\frac{\rho_{n} -
		 \rho_{p}}{\rho}\right) ,
\]
from section (\ref{asym}), the energy density need to be expressed in terms of $t$. This can be done by considering the expression for the proton ($\rho_p$), neutron ($\rho_n$) and baryon ($\rho$) number densities. These are given as in terms of the different fermi momenta of the species
\begin{eqnarray}
	\rho_p &=& \frac{1}{\pi^{2}}\int^{k_{p}}_{0}dk\,k^{2} = \frac{k_p^3}{3\pi^2},\nonumber\\
	\rho_n &=& \frac{1}{\pi^{2}}\int^{k_{n}}_{0}dk\,k^{2} = \frac{k_n^3}{3\pi^2},\nonumber\\ \rho &=& \rho_p + \rho_n\nonumber.
\end{eqnarray}
In the case of symmetric nuclear matter ($t = 0$) the proton and neutron fermi momenta are equal, $k_p$ = $k_n$ = $k_f$, and the baryon density reduced to
\begin{eqnarray}
	\rho_0 = 2 \times \frac{1}{\pi^{2}}\int^{k_{f}}_{0}dk\,k^{2} = \frac{2k_f^3}{3\pi^2}\,\,.\label{rho0}
\end{eqnarray}
%\begin{center}
To evaluate the expression for the symmetry energy the proton and neutron fermi momenta must be expressed in terms of $t$, i.e.
\begin{eqnarray}
	k_n &=& \left[3\pi^2\frac{1}{2}\frac{kp^3 + k_n^3}{3\pi^2}(1 + t)\right]^\frac{1}{3}\nonumber\\
			&=&  \left[\frac{k_p^3 + k_n^3}{2}(1 + t)\right]^\frac{1}{3}\label{kn}
\end{eqnarray}
and
\begin{eqnarray}
	k_p &=& \left(3\pi^2\frac{1}{2}\frac{kp^3 + k_n^3}{3\pi^2}(1 - t)\right)^\frac{1}{3}\nonumber\\
			&=&  \left(\frac{k_p^3 + k_n^3}{2}(1 - t)\right)^\frac{1}{3}\,.\label{kp}
\end{eqnarray}
The only terms in the expression of the energy-density (\ref{eps}) that will contribute are the integrals over the filled baryon states. Thus the expression for $a_4$ is
\[
		a_{4} = \frac{1}{2}\left.\frac{\partial^{2}}{\partial t^{2}}
		\left(\frac{1}{\rho}\frac{1}{\pi^{2}}\int^{k_{n}}_{0}dk\,k^{2}\sqrt{k^{2} + {m^{*}}^{2}} + 
		\frac{1}{\rho}\frac{1}{\pi^{2}}\int^{k_{p}}_{0}dk\,k^{2}\sqrt{k^{2} + {m^{*}}^{2}}\right)\right|_{t=0},
\]
which reduces to 
\begin{eqnarray}
		a_{4} = \frac{k_f^2}{6(k_f^2 + m^{*2})^\frac{1}{2}}
\end{eqnarray}
after substituting in the expressions for the different fermi momenta,(\ref{kn}), (\ref{kp}) and keeping in mind (\ref{rho0}) at the evaluation point as well as some algebra.

\textbf{\huge\texttt{sit QHD1 se resultate in}}
%
%
%
\begin{eqnarray}
\epsilon &=&   \frac{1}{2}m_s^{2}\phi_0^{2} + \frac{\kappa}{3!}(g_s\phi_0)^3 + \frac{\lambda}{4!}(g_s\phi_0)^4 - \frac{1}{2}m_\omega^{2}V_{0}^2
	 - \frac{\zeta}{4!}g_v^4V_0^4 - \frac{1}{2}m_{\rho}^{2}b_0^2 - \Lambda_vg_v^2V_0^2 g_\rho^2b_0^2 \\\nonumber
	 &+& g_vV_0(\rho_n + \rho_p) + \frac{1}{2}g_\rho b_0(\rho_p - \rho_n) + eA_0\rho_p +
	 \frac{1}{\pi^{2}}\int^{k_{p}}_{0}dk\,k^{2}\sqrt{k^{2}+{m^{*}}^{2}}\\\nonumber
	  &+& \frac{1}{\pi^{2}}\int^{k_{n}}_{0}dk\,k^{2}\sqrt{k^{2}+{m^{*}}^{2}}\\\nonumber
	 \end{eqnarray}
	 %\\\nonumber
	 \begin{eqnarray}
	p = - \frac{1}{2}m_s^{2}\phi_0^{2} - \frac{\kappa}{3!}(g_s\phi_0)^3 - \frac{\lambda}{4!}(g_s\phi_0)^4 + \frac{1}{2}m_\omega^{2}V_{0}^2
	 + \frac{\zeta}{4!}g_v^4V_0^4 + \frac{1}{2}m_{\rho}^{2}b_0^2 + \Lambda_vg_v^2V_0^2 g_\rho^2b_0^2 \\\nonumber
	 \frac{1}{3\pi^{2}}\int^{k_{p}}_{0}dk\,\frac{k^{4}}{\sqrt{k^{2}+{m^{*}}^{2}}} + 
	 \frac{1}{3\pi^{2}}\int^{k_{n}}_{0}dk\,\frac{k^{4}}{\sqrt{k^{2}+{m^{*}}^{2}}}\\
\end{eqnarray}

%\end{center}
	
\begin{eqnarray}
	\epsilon_s = - \frac{1}{2}m_{\rho}^{2}b_0^2 - \Lambda_vg_v^2V_0^2 g_\rho^2b_0^2  
	+ \frac{1}{2}g_\rho b_0(\rho_p - \rho_n) + eA_0\rho_p \\\nonumber
	+ \frac{1}{\pi^{2}}\int^{k_{p}}_{0}dk\,k^{2}\sqrt{k^{2}+{m^{*}}^{2}} + 
	 \frac{1}{\pi^{2}}\int^{k_{n}}_{0}dk\,k^{2}\sqrt{k^{2}+{m^{*}}^{2}}\\\nonumber
	 \\\nonumber
	 g_{\rho}b_0 =
		 \frac{g_\rho^2}{m_\rho^2}\left[\frac{1}{2}\left\langle\psi^\dagger\tau_3\psi\right\rangle - 
		 2\Lambda_v(g_vV_0)^2(g_\rho b_0)\right]\\
		 = \frac{g_\rho^2}{m_\rho^2}\left[\frac{1}{2}(\rho_p - \rho_n) - 
		 2\Lambda_v(g_vV_0)^2(g_\rho b_0)\right]\\
\end{eqnarray}

%
%
%
%
%
%
\section{Advanced models}
Field theory description of nuclei and nuclear matter has undergone various improvements. These include self-couplings of the $\sigma$-field introduced by Boguta and Bodmer {\bfseries(sit ref in !!!!)} to give a better description of the nuclear compressibility etc\\
\\
{\bf brei verder ook uit hier, sit miskien sat prop nuclei ook hier in en se hoekom belangrik, want dit motiveer ook verstelling en verdere modelle. of maak aparte hoofstuk oor matter prop en hoe verbeter het binne ander models - ook wat die delta tussen die modelle...}\\
\\
The most general Lagrangian, that descibes the QHD1, NL3, NL-SH, FSUGold, PK1, TM1 and TM2 relativistic field theory models for nuclei and nuclear matter, where the isodoublet nucleon field $\psi$ interacting via the exchange of one scalar field, $\phi$ and three vector ($V^\mu$ for the omega, ${\bf b}^\mu$ for the rho and $A^\mu$ for the photon) fields, is
\begin{eqnarray}\label{fsuglagrangian}
			{\cal L} &=& \bar{\psi}(x)[\gamma^{\mu}(i\partial_{\mu} - g_{v}V_{\mu}) - \frac{g_\rho}{2}{\bm\tau}\cdot{\bf b}_\mu
			- \frac{e}{2}(1 + \tau_3)A_\mu - (M-g_{s}\phi)]\psi(x) \\\nonumber
			&+& \frac{1}{2}\partial_{\mu}\phi\partial^{\mu}\phi - \frac{1}{2}m_s^{2}\phi^{2} 
			- \frac{\kappa}{3!}(g_s\phi)^3 - \frac{\lambda}{4!}(g_s\phi)^4 \\\nonumber
			&-& \frac{1}{4}V^{\mu\nu}V_{\mu\nu} + \frac{1}{2}m_\omega^{2}V^{\mu}V_{\mu} + 
			\frac{\zeta}{4!}(g_v^2V^\mu V_\mu)^2 + \Lambda_vg_v^2V^\mu V_\mu g_\rho^2\textbf{b}^{\mu}\cdot\textbf{b}_{\mu}\\\nonumber
			&-& \frac{1}{4}\textbf{b}^{\mu\nu}\textbf{b}_{\mu\nu} + \frac{1}{2}m_{\rho}^{2}\textbf{b}^{\mu}\cdot\textbf{b}_{\mu} \\\nonumber
			&-& \frac{1}{4}F^{\mu\nu}F_{\mu\nu}
			%\\
		%
		%
%		\begin{array}[h]{l}
%			{\cal L} = \bar{\psi}[\gamma^{\mu}(i\partial_{\mu} - g_{v}V_{\mu}) - \frac{g_\rho}{2}{\bm \tau}\cdot{\bf b}_\mu
%			- \frac{e}{2}(1 + \tau_3)A_\mu - (M-g_{s}\phi)]\psi \\
%			\\
%			+ \frac{1}{2}\partial_{\mu}\phi\partial^{\mu}\phi - \frac{1}{2}m_s^{2}\phi^{2} 
%			- \frac{\kappa}{3!}(g_s\phi)^3 - \frac{\lambda}{4!}(g_s\phi)^4 \\
%			\\
%			- \frac{1}{4}V^{\mu\nu}V_{\mu\nu} + \frac{1}{2}m_\omega^{2}V^{\mu}V_{\mu} + 
%			\frac{\zeta}{4!}(g_v^2V^\mu V_\mu)^2 + \Lambda_vg_v^2V^\mu V_\mu g_\rho^2\textbf{b}^{\mu}\cdot\textbf{b}_{\mu}\\
%			\\
%			- \frac{1}{4}\textbf{b}^{\mu\nu}\textbf{b}_{\mu\nu} + \frac{1}{2}m_{\rho}^{2}\textbf{b}^{\mu}\cdot\textbf{b}_{\mu} \\
%			\\
%			- \frac{1}{4}F^{\mu\nu}F_{\mu\nu}
%		\end{array}
\end{eqnarray}	
where the field tensors have been defined as
\begin{eqnarray}
	V_{\mu\nu} = \partial_\mu V_\nu - \partial_\nu V_\mu\\
	\textbf{b}_{\mu\nu} = \partial_\mu\textbf{b}_{\nu} - \partial_\nu\textbf{b}_{\mu}\\
	F_{\mu\nu} = \partial_\mu A_\nu - \partial_\nu A_\mu,
\end{eqnarray}
with
\begin{itemize}
	\item $e$ the electron charge, and
	\item ${\bm \tau} = (\tau_1, \tau_2, \tau_3)$ the isospin operater. This operator given in terms of the Pauli 2$\times$2 spin-matrices
	 (\ref{pauli-spin}) as
		\[
			{\bm \tau}  = \left[
											\begin{array}{cc}
												{\bm \sigma} & 0\\
												0 & {\bm \sigma}				 
											\end{array}	
										\right].		
		\]
		It should be noted that since the nucleon field, $\psi$ is an isodoublet and therefore
		\[
			\psi = \left[
											\begin{array}{c}
												\psi_p\\
												\psi_n				 
											\end{array}	
										\right]\footnote{see \ref{conventions}},
		\]
		where is the $\psi_p$ is the proton field and $\psi_n$ is the neutron field, each consisting of the 4$\times$1 Dirac spinors, that the 				total dimension of $\psi$ is 8$\times$1. Therefore $\tau$ is in actual fact given by
	%	\[	
	%			\begin{table}{rcccl}[h]
	%				\centering
	%					\begin{tabular}
	%						${\bm \tau}$ & = & $\left[\begin{array}{cc}{\bm \sigma}$ & 0\\0 & ${\bm \sigma}\end{array}\right]$&$\otimes$&
	%						$\left[\begin{array}{cc} 1_4$& 0\\0&$1_4$\end{array}\right]$.	
	%					\end{tabular}
	%			\end{table}											
	%	\]
			\begin{eqnarray}
				\begin{tabular}{rcccl}
										${\bm \tau}$ & = &
											$\left[\begin{array}[h]{cc}{\bm \sigma} & 0\\0 & {\bm \sigma}\end{array}\right]$& $\otimes$ 
											&$\left[\begin{array}[h]{cc}\textbf{1}_4 & 0\\0 & \textbf{1}_4\end{array}\right]$.	
				\end{tabular}\\
				{\bm \tau} = {\bm \sigma} \otimes \left[\begin{array}[h]{cc}\textbf{1}_4 & 0\\0 & \textbf{1}_4\end{array}\right]
			\end{eqnarray}
			and therefore the explicit expression for $\tau_3$ is
			\begin{eqnarray}
				\tau_3 
				= \left[\begin{array}[h]{cc}1 & 0\\0 & -1\end{array}\right] \otimes 
				\left[\begin{array}[h]{cc}\textbf{1}_4 & 0\\0 & \textbf{1}_4\end{array}\right]   
				= \left[\begin{array}[h]{cc}\textbf{1}_4 & 0\\0 & -\textbf{1}_4\end{array}\right] 
				= \left[\begin{array}[h]{cccccccc}1 & 0&0&0&0&0&0&0\\0 & 1&0&0&0&0&0&0\\0 & 0&1&0&0&0&0&0\\0 & 0&0&1&0&0&0&0\\
				0&0&0&0&-1&0&0&0\\0&0&0&0&0&-1&0&0\\0&0&0&0&0&0&-1&0\\0&0&0&0&0&0&0&-1\\\end{array}\right]\nonumber
			\end{eqnarray}
\end{itemize}
Since all terms contract the Lagrangian is still a Lorentz scalar and thus can be applied in the framework of Special Relativity {\sl\textbf{maak seker van wat jy hier se en sorg dat binne algemene Spes rel en field theory gedef is}}. The Lagrangian has the dimension of fm$^{-4}$.\\
\\
Using the Euler-Lagrange equation the equations of motion of the different fields can be calculated.
\begin{eqnarray}\label{EQM}
		\partial_{\mu}\partial^{\mu}\phi + m_s^{2}\phi + \frac{\kappa}{2!}g_s^3\phi^2 + \frac{\lambda}{3!}g_s^4\phi^3  = 		
		g_{s}\bar{\psi}(x)\psi(x)\nonumber\\
		%
		\partial_{\mu}V^{\mu\nu} + m_\omega^{2}V^{\nu} + \frac{\zeta}{3!}g_v^4V_\nu^2 V^\nu + 
		2\Lambda_vg_v^2V^\nu g_\rho^2\textbf{b}^{\mu}\cdot\textbf{b}_{\mu}= g_{v}\bar{\psi}(x)\gamma^{\nu}\psi(x)\nonumber\\
		%
		\partial_{\mu}\textbf{b}^{\mu\nu} + m_{\rho}^{2}\textbf{b}^{\nu} + 2\Lambda_vg_v^2V^\nu V_\nu g_\rho^2\textbf{b}^\nu=
		 \frac{g_\rho}{2}\bar{\psi}(x)\gamma^{\nu}\vec\textbf{$\tau$}\psi(x)\nonumber\\
		%
		\partial_{\mu}F^{\mu\nu} = g_{v}\bar{\psi}(x)\gamma^{\nu}\frac{e}{2}(1 + \tau_3)\psi(x)\nonumber\\
		%
		(\gamma^{\mu}(i\partial_{\mu}-g_{v}V_{\mu} - \frac{g_\rho}{2}{\bm \tau}\cdot{\bf b}_\mu
		- \frac{e}{2}(1 + \tau_3)A_\mu) - (M-g_{s}\psi))\psi(x) = 0.
		%\\
		%
			%
			%
%		\begin{array}[h]{l}
%					\partial_{\mu}\partial^{\mu}\phi + m_s^{2}\phi + \frac{\kappa}{2!}g_s^3\phi^2 + \frac{\lambda}{3!}g_s^4\phi^3  =
%					 g_{s}\bar{\psi}\psi\\
%					 \\
%					\partial_{\mu}V^{\mu\nu} + m_\omega^{2}V^{\nu} + \frac{\zeta}{3!}g_v^4V_\nu^2 V^\nu + 
%					2\Lambda_vg_v^2V^\nu g_\rho^2\textbf{b}^{\mu}\cdot\textbf{b}_{\mu}= g_{v}\bar{\psi}\gamma^{\nu}\psi\\
%					\\
%					(\gamma^{\mu}(i\partial_{\mu}-g_{v}V_{\mu} - \frac{g_\rho}{2}{\bm \tau}\cdot{\bf b}_\mu
%						- \frac{e}{2}(1 + \tau_3)A_\mu) - (M-g_{s}\psi))\psi = 0
%						\\
%		\end{array}		
\end{eqnarray}
%
%
%
%
\subsection{Conventions}\label{conventions}
There are two different conventions for expressing the Lagrangian. These differences are obvious when the Lagrangian and the value of the coupling constants of the NL3 model in Ref. \cite{Todd} are compared to that of Ref. \cite{NL3}.\\
\\
The way in which the Lagrangian (\ref{fsuglagrangian}) is expressed will be refered to as the \emph{American} convention. This convention is the original formulation of the Walecka-type relativistic field theory models of the nucleus (see Ref. \cite{walecka}). The other convention of expressing the Lagrangian is mainly used by authors from Europe and the Orient. This formulation will be refered to as the \emph{Oriental} convention.\\
\\
The difference is that in the Western convention the scalar field $\phi$ is explicitly positive, where as in the Oriental convention it is negative. The first four components in the nucleon field $\psi$ of the American convention refers to the proton field and the last four to neutron field whereas in the Oriental convention the first four componenets of the nucleon field refers to the neutron field and the last four to the proton field. In the Western convention the coupling between the rho-field, ${\bf b}_\mu$ and the iso-spin density, $g_\rho$ has an explicit factor of a half and in the Oriental convention this factor is implied. \\
\begin{table}[htb]
	\centering
		\begin{tabular}{ccc}
			\hline\\
			\hline\\
			Property & Western & Oriental\\
			\hline\\
			Reduced nucleon mass (m$^*$)& $m^* = M - g_s\phi$& $m^* = M + g_s\phi$\\
			\\
			Coupling between the rho-field and \\nucleon fields, $g_\rho$ & $\bar{\psi}\gamma^\mu\frac{g_\rho}{2}{\bm \tau}\cdot{\bf b}_\mu\psi$ & 
			$\bar{\psi}\gamma^\mu g_\rho{\bm \tau}\cdot{\bf b}_\mu\psi$\\
			\\
			Third-order self-coupling constant \\in the scalar-meson field & $\kappa$ & $g_2$\\
			\\
			Fourth-order self-coupling constant \\in the scalar-meson field & $\lambda$ & $g_3$\\
			\\
			Self-coupling constant in the omega-\\meson field & $\zeta$ & $c_3$\\
			\\
			Coupling between the rho- and the omega-\\meson fields & $\Lambda_v$ & Not applicable\\
			\\
			Nucleon field $\psi$ & $\psi = \left[\begin{array}{c}\psi_p\\\psi_n\end{array}\right]$ & 
			$\psi = \left[\begin{array}{c}\psi_n\\\psi_p\end{array}\right]$\\
			\\
			\hline
		\end{tabular}
	\caption{Differences in Western and Oriental expressions of the Lagrangian of relativistic field theory models for nuclear matter.}
	\label{tab:convention}
\end{table}
\\
In this work the American convention will be used. Oriental expression for certain properties will also be given but identified as such. Both conventions are included for the different relativistic field theory models are studied within the specific context that they were defined. It should also be noted that while certain terms will be present in one convention it might not be the other. This due to the fact that different relativistic field theory models included different couplings and as such certain couplings might only be used in models studied by authors of a specific convention.\\
\\
It should also be noted the coupling constants are defined seperately for each convention.\\
\\
The differences between the two conventions is contrasted in Table \ref{tab:convention}.
%
%
%
%
%
\subsection{Mean-field equations}
As in section (\ref{QHD1}) the equations of motion for the different fields are solved in the relativistic mean-field approximation, which for a uniform, static, spherical symmetric system implies the fields are replaced by their expectation values,
\begin{eqnarray}\nonumber
		\phi(x) \longrightarrow \left\langle \phi(x)\right\rangle = \phi_{0}\\\nonumber
		\omega^{\mu}(x) \longrightarrow \left\langle \omega^\mu(x)\right\rangle = g^{\mu 0}\omega_{0}\\\nonumber
		{\bf b}^{\mu}(x) \longrightarrow \left\langle b^{\mu}_a(x)\right\rangle = g^{\mu 0}\delta_{a3}b_0^a\\\nonumber
		A^{\mu}(x) \longrightarrow \left\langle A^{\mu}(x)\right\rangle = g^{\mu 0}A_0\nonumber
\end{eqnarray}
and the baryon sources must be replaced by their normal-order expectation values in the mean-field grondstate,
\begin{eqnarray}\nonumber
	\bar\psi(x){\bf 1}\psi(x) \longrightarrow \left\langle :\bar\psi(x){\bf 1}\psi(x):\right\rangle = \rho_s\\\nonumber
	\bar\psi(x)\gamma^\mu\psi(x) \longrightarrow \left\langle :\bar\psi(x)\gamma^\mu\psi(x):\right\rangle = g^{\mu0}\rho_v\\\nonumber
	\bar\psi(x)\gamma^\mu\tau_a\psi(x) \longrightarrow \left\langle :\bar\psi(x)\gamma^\mu\tau_a\psi(x):\right\rangle = 
	g^{\mu0}\delta_{a3}\rho_3\\\nonumber
	\bar\psi(x)\gamma^\mu(\frac{1 + \tau_3}{2})\psi(x) \longrightarrow 
	\left\langle :\bar\psi(x)\gamma^\mu(\frac{1 + \tau_3}{2})\psi(x):\right\rangle = g^{\mu0}\delta_{a3}\rho_p. \nonumber
\end{eqnarray}
In the mean-field approximation the equations of motion (\ref{EQM}) of the fields reduce to:
\begin{eqnarray}
		g_s\phi_0 = \frac{g_{s}^2}{m_s^2}\left[\left\langle\bar\psi\psi\right\rangle - 
		\frac{\kappa}{2}(g_s\phi_0)^2 - \frac{\lambda}{6}(g_s\phi_0)^3\right]\\
		%
		g_{v}V_0 = \frac{g_{v}^2}{m_\omega^2}\left[\left\langle \psi^{\dagger}\psi\right\rangle - \frac{\zeta}{6}(g_vV_0)^3 - 
		2\Lambda_v(g_vV_0)(g_\rho b_0)^2\right]\\
		%
		g_{\rho}b_0 =
		 \frac{g_\rho^2}{m_\rho^2}\left[\frac{1}{2}\left\langle\psi^\dagger\tau_3\psi\right\rangle - 
		 2\Lambda_v(g_vV_0)^2(g_\rho b_0)\right]\\
		 %
		\left[i\gamma^{\mu}\partial_{\mu}-g_{v}\gamma^0V_{0} - \frac{g_\rho}{2}\tau_3\gamma^0b_0
		- \frac{e}{2}(1 + \tau_3)\gamma^0 A_0 - (M-g_{s}\psi)\right]\psi = 0
\end{eqnarray}	
In the Oriental convention\footnote{The coupling between the rho- and the omega-meson fields, $\Lambda_v$, are not included in any model studied within the Oriental convention.} these equations are given by:
\begin{eqnarray}
		m_s^2\phi_0 = -g_s\left\langle\bar\psi\psi\right\rangle -g_2\phi_0^2 - g_3\phi_0^3\\
		%
		m_\omega^2V_0 = g_v\left\langle \psi^{\dagger}\psi\right\rangle - c_3 V_0^3\\
		%
		m_{\rho}^2b_0 =g_\rho\left\langle\psi^\dagger\tau_3\psi\right\rangle\\
		 %
		\left[i\gamma^{\mu}\partial_{\mu}-g_{v}\gamma^0V_{0} - g_\rho\tau_3b_0
		- \frac{e}{2}(1 - \tau_3)A_0 - (M+g_{s}\psi)\right]\psi = 0
\end{eqnarray}
%
%
%
%
%\newpage
\subsection{Coupling constants and masses}
Each model studied in this work is defined by a unique set of parameters, that gives the values of the coupling constants and masses that should be used. In relativistic field theory models the coupling constants are determined by fitting calculated properties of nuclear matter (as discussed in (\ref{satprop})) to that of the experimentally determined values. Once these values are determined, they are fixed for all calculations done within the model.\\
\\
{\sl\textbf{kan iets se van density dependant couplings en oor hoe mcoupln=ings bereken word...?}}\\
\\
{\sl\textbf{moet verskillende modelle ook nie hier beskryf word nie???}}\\
\\
The paramaters for the QHD1 calculations done in this work are those given by Serot and Walecka in Ref.\cite{recentprogress}.\\
The Oriental NL3 parameters are taken from the original article by Lalazissis \textsl{et al.} \cite{NL3}, while the parameters in the Western convention are from Ref. \cite{Todd}.\\
The parameters for the PK1 model are taken from the article by Long \textsl{et al.} \cite{PK1}, while the paramater set of NL-SH and TM1 (as well as TM2) are taken from the article by Sharma and Nagarajan \cite{NLSH} and the article by Sugahara and Toki \cite{TM1}, respectively.\\
The parameters for the FSUGold model and the NL3 parameters in the Western convention are given by Todd-Rutel and Piekarewicz in Ref. \cite{Todd}. \\
\\
The values for the coupling constants and masses for models studied in the Western convention are given in Table (\ref{tab:westcoupling}) and Table(\ref{tab:westmasses}) respectively, while those for the Oriental convention are given in Table (\ref{tab:orientcoupling}) and Table (\ref{tab:orientmasses}).

\begin{table*}[htb]
	\centering
		\begin{tabular}{cccccccc}
			\hline\\
			\hline\\
			Model & $g_s^2$ & $g_v^2$ & $g_\rho^2$& $\kappa$(MeV) & $\lambda$ & $\zeta$ & $\Lambda_v$ \\
			\hline\\
			NL3  & 104.3871 & 165.5854 & 79.6000 & 3.8599 & -0.01591 & 0.00 & 0.00 \\
			S271  & 81.1071  & 116.7655 & 85.4357 & 6.6834 & -0.01580 & 0.00 & 0.00 \\
			Z271&  49.4401  & 70.6689  & 90.2110 & 6.1696 & +0.15634 & 0.06 & 0.00 \\
			FSUGold & 112.1996 & 204.5469 & 138.4701& 1.4203 & +0.0238  & 0.0600 & 0.0300 \\
			\hline
		\end{tabular}
	\caption{Coupling constants for different models defined in the Western convention. All coupling constants are dimensionless, except 
	$\kappa$ which is given in MeV.}
	\label{tab:westcoupling}
\end{table*}

\begin{table*}[hbt]
	\centering
		\begin{tabular}{cccccc}
			\hline\\
			\hline\\
			Model & $M_{\mbox{\footnotesize{proton}}}$& $M_{\mbox{\footnotesize{neutron}}}$& $m_s$& $m_\omega$& $m_\rho$ \\
			\hline\\
			NL3 & 939 & 939 & 508.1940 & 782.5  & 763\\
			S271 & 939 & 939 & 505.000 & 783  & 763\\
			Z271&939 & 939 & 465.000 & 783  & 763\\
			FSUGold & 939 & 939 & 491.5000 & 783  & 763\\
			\hline
		\end{tabular}
	\caption{Particle masses (in MeV) for models defined in the Western convention.}
	\label{tab:westmasses}
\end{table*}

\begin{table*}[htb]
	\centering
		\begin{tabular}{ccccccc}
			\hline\\
			\hline\\
			Model & $g_s$ & $g_v$ & $g_\rho$& $g_2$(fm$^{-1}$) & $g_3$ & $c_3$ \\
			\hline\\
			NL3 & 10.217 & 12.868 & 4.474 & -10.431 & -28.885 & 0.00\\
			PK1  & 10.3222 & 13.0131 & 4.5297 & -8.1688 & -9.9976 & 55.636\\
			TM1 & 10.0289 & 12.6139 & 4.6322 & -7.2325 & 0.6183 & 71.3075\\
			TM2 & 11.4694 & 14.6377 & 4.6783 & -4.4440 & 4.6076 & 84.5318\\
			NL-SH  & 10.444 & 12.945 & 4.383 & -6.9099 & -15.8337 & 0.00\\
			
			\hline
		\end{tabular}
	\caption{Coupling constants for different models defined in the Oriental convention. All coupling constants are dimensionless, 
	except $g_2$ which is given in fm$^{-1}$.}	\label{tab:orientcoupling}
\end{table*}

\begin{table*}[hbt]
	\centering
		\begin{tabular}{cccccc}
			\hline\\
			\hline\\
			Model & $M_{\mbox{\footnotesize{proton}}}$& $M_{\mbox{\footnotesize{neutron}}}$& $m_s$& $m_\omega$& $m_\rho$ \\
			\hline\\
			NL3 & 939 & 939 & 508.194 & 782.501  & 763.0000\\
			PK1  & 939.5731 & 938.2796 & 514.0891 & 784.254 & 763\\
			TM1  & 938 & 938 & 511.198 & 783.0 & 770.0\\
			TM2  & 938 & 938 & 526.443 & 783.0 & 770.0 \\
			NL-SH  & 939 & 939 & 526.059 & 783.00 & 763.00\\
			
			\hline
		\end{tabular}
	\caption{Particle masses (in MeV) for models defined in the Oriental convention.}
	\label{tab:orientmasses}
\end{table*}

%
%
%
\subsection{Equation of state}
\subsection{Nuclear matter observables}
\subsubsection{Symmetry energy}
The symmerty energy coeffiecient for the advanced models are calculated in exactly the same way as for QHD1, except that the energy density in the advanced models has more isospin dependant terms.\\
\\
The general expression for the energy density ()
















%
%
%
%
%
%
